The First Reactive Synthesis Competition (SYNTCOMP 2014)

We introduce the reactive synthesis competition (SYNTCOMP), a long-term effort intended to stimulate and guide advances in the design and application of synthesis procedures for reactive systems. The first iteration of SYNTCOMP is based on the controller synthesis problem for finite-state systems and safety specifications. We provide an overview of this problem and existing approaches to solve it, and report on the design and results of the first SYNTCOMP. This includes the definition of the benchmark format, the collection of benchmarks, the rules of the competition, and the five synthesis tools that participated. We present and analyze the results of the competition and draw conclusions on the state of the art. Finally, we give an outlook on future directions of SYNTCOMP.

==> abssynthe.tex <==
\subsection{AbsSynthe: an abstract synthesis tool}
%\subsubsection{Introduction}
%\paragraph{Input of the Algorithm}
%AbsSynthe takes as input a safety specification described by a file in the
%\emph{extended AIGER format}~\cite{jacobs14}.
%The original AIGER format~\cite{aiger} is a
%safety property specification used for model checking purposes. The extended
%version of it has been recently introduced by Jacobs~\cite{jacobs14} as a
%standard way of representing safety objectives for controller synthesis.

AbsSynthe was submitted by R. Brenguier, G. A. P\'erez, J.-F. Raskin, and 
O. Sankur from Universit\'e Libre de Bruxelles. AbsSynthe implements a 
BDD-based synthesis approach in Python, with the following optimizations:
\begin{itemize}
\item partitioned transition relation
\item automatic BDD reordering \sj{details?}
\item direct substitution of state variables with BDDs
\item strategy extraction based on XXX
\item optional: abstraction method
\item optional: minimization of synthesized circuit by forward reachability analysis
\end{itemize}

AbsSynthe is described in more detail in~\cite{BrenguierPRS14}. 
AbsSynthe competed in all subtracks, and was intended to compete in different 
configurations, some of which 
include the optional optimizations above. Due to a miscommunication between 
tool authors and competition organizers, the necessary parameters were not 
used, such that only the basic configuration participated. Sadly, this error
was discovered too late to run the additional configurations before the 
presentation of results at CAV 2014. However, as mentioned
in~\cite{BrenguierPRS14}, the abstraction-based method overall performed
worse than the standard method, and thus the fastest configuration did 
participate in the competition. For completeness, we show the comparison of
benchmark results for different versions of \abssynthe in
Figure~\ref{fig:real-sorted}.
\sj{detail: launch commands were not provided correctly in the EDACC system 
by tool authors. different submitted configurations differed in source code, 
and could be started with identical launch command. However, to correctly 
start the different configurations, different launch commands were also 
needed.}

% \subsubsection{Abstract algorithm}
%  \sj{should be significantly shortened}
% Let $P$ be a set of boolean variables, which we will call \emph{predicates}.
% Each $p \in P$ has an associated boolean formula $f_p(L)$. $P$ contains a
% predicate $p_I$ which holds if and only if all latches are set to $0$ and a
% predicate $p_U$ which holds if and only if $\out$ is set to $1$. 
% %corresponds to $\mathcal{U}$ (see previous subsection).

% We define the \emph{concretization function} $\gamma : \pow(Q^\abs) \to
% \pow(Q)$ as 
% \[
% \gamma(S^\abs)(L) = S^\abs(P)[p \leftarrow f_p(L)]_{p \in P}.
% \]
% The dual operation is abstraction; we define two \emph{abstraction functions}
% $\overline{\alpha}, \underline{\alpha} : \pow(Q) \to \pow(Q^\abs)$ as follows:
% \[
% 	\overline{\alpha}(S)(P) = \exists L: S(L) \land (\bigwedge_{p \in P} p
% 	\Leftrightarrow f_p(L)),
% \]
% \[
% 	\underline{\alpha}(S) = \exists L: \lnot (\lnot S(L) \land (\bigwedge_{p
% 	\in P} p \Leftrightarrow f_p(L))).
% \]

% We define over and under approximations of $\upre$ which operate on valuations
% of $P$. Let $\psi_p(L,X_u,X_c) = f_p(L')[l' \leftarrow f_l(X_u,X_c,L)]_{l \in
% L}$.  Then the $\upreover(S^\abs),\upreunder(S^\abs)$ operators can be computed
% as shown below.
% \[
% 	\exists X_u.\ \forall X_c : \overline{\alpha}(S^\abs(P')[p'
% 		\leftarrow \psi_p(X_u,X_c,L)]_{p \in P})
% \]
% \[
% 	\lnot (\forall X_u.\ \exists X_c :
% 		\overline{\alpha}(\lnot S^\abs(P')[p' \leftarrow \psi_p(X_u,X_c,L)]_{p \in
% 		P})),
% \]
% where $S^\abs$ is a boolean formula over $P$. We will also need an operator to
% compute abstract states reachable when environment is playing in a certain
% fashion. To this end, given a boolean formula $\qstratadam(P,X_u)$ which defines
% a relation between predicate and uncontrollable inputs, we define the
% $\post(S^\abs, \qstratadam)$ operator below
% \begin{align*}
% 	\exists L, X_u, X_c :& (S^\abs(P) \land
% 	\qstratadam(P,X_u))[p \leftarrow f_p(L)]_{p \in P} \land\\
% 	&\bigwedge_{p \in P} p' \Leftrightarrow \psi_p(X_u,X_c,L).
% \end{align*}
% In our implementation we chose to over-approximate $\post$. We denote by
% $\overline{\post}$ the result of pushing the quantification over $X_c$ after
% $\bigwedge_{p \in P}$. 

% %We also need to define an operator which yields, given a boolean formula
% %$S^\abs$ over $P$ and a boolean formula $\qstratadam(P,X_u)$, an
% %over-approximation of the configurations that can be reached.
% %Formally, we define $\overline{\post}(S^\abs, \qstratadam)$ as
% %\begin{align*}
% %	\exists L, X_u :& (S^\abs(P) \land
% %	\qstratadam(P,X_u))[p \leftarrow f_p(L)]_{p \in P} \land\\
% %	&\bigwedge_{p \in P} \exists X_c: p' \Leftrightarrow \psi_p(X_u,X_c,L).
% %\end{align*}

% \paragraph{Algorithm.}
% On the one hand, if the fixpoint of the under-approximated operator contains the
% initial configuration, we are certain that the specification is unrealizable. On
% the other hand, if the fixpoint of the over-approximated operator does not
% contain the initial configuration, we know that the specificaiton is realizable.
% %Since the operators
% %are not exact,
% The converse of the above assertions does not hold. In this case
% we add aditional predicates (in practice, we apply \emph{localization
% reduction}~\cite{kurshan94}) to our model in order to have a finer abstraction.

% \begin{algorithm}
% 	\small
% 	$W_u$ := $\mu X .\ (\mathcal{U}^\abs \cup
% 		\upreunder(X)) \cap R^\abs$\;
% 	\uIf{$q_I^\abs \in W_u$}
% 	{
% 		\Return not controllable\;
% 	}
% 	\Else
% 	{
% %		$R^\abs$ := $R^\abs$\;
% 		$prev$ := $\emptyset$\;
% 		\While{$R^\abs \neq prev$}
% 		{
% 			$prev$ := $R^\abs$\;
% 			$W_o$ := $\mu X .\ (W_u \cup
% 				\upreover(X)) \cap R^\abs$\;
% 			\eIf{$q_I^\abs \not\in W_o$}
% 			{
% 				\Return controllable\;
% 			}
% 			{
% %				\tcc{strategy and post operators are abstract}
% 				$\qstratadam$ := quasi-strategy defined by $(W_o)$\;
% 				$R^\abs$ := $\mu X .\ (q^\abs_I \cup
% 					\overline{\post}(X, \qstratadam)) \cap R^\abs$\;
% 			}
% 		}
% 		$W'_u$ := $(\upre_\cqstratadam(\gamma(W_u)))
% 			\cap \gamma(R^\abs)$\;
% 		\eIf{$W'_u \subseteq \gamma(W_u)$}
% 		{
% 			\Return controllable\;
% 		}
% 		{
% %			\tcc{call \texttt{add\_pred} and \texttt{loc\_red}}
% 			$Q^\abs_2$ := \texttt{refine}$(Q^\abs, W'_u \cup
% 				\gamma(W_u), \gamma(R^\abs))$\;
% 			\tcc{$\underline{\alpha}_2,\overline{\alpha}_2$ are the associated
% 			abstraction operators}
% 			$\mathcal{U}^\abs_2$ := $\underline{\alpha}_2(W'_u \cup
% 				\gamma(W_u))$\;
% 			\Return \texttt{abs\_synth}$(G, G^\abs_2,
% 			\overline{\alpha}_2(\gamma(R^\abs)))$\;
% 		}
% 	}
% \caption{\texttt{abs\_synth}$(G, G^\abs, R^\abs)$}
% \label{alg:abs_synth}
% \end{algorithm}

% We now outline the main stages of Algorithm~\ref{alg:abs_synth}.
% \begin{enumerate}
% 	\item Add to $P = \{p_I,p_U,p_R\}$, where $p_R \equiv 1$, some
% 		additional predicates each of which hold if and only if a latch
% 		holds (i.e. $\{p_l \:\mid \: p_l \Leftrightarrow l$ and $ l \in
% 		\mathcal{L}\}$ for some $\mathcal{L} \subseteq L$).
% 	\item If $W_u \ni p_I$, the specification is
% 		unrealizable.
% 	\item Repeat the following until $p_R$ is not updated:
% 		\begin{enumerate}
% 			\item If $W_o \not\ni p_I$, then
% 				the specification is realizable;
% 			\item otherwise, we extract a boolean formula
% 				$\qstratadam(P,X_u)$, which
% 				corresponds to a relation that chooses $X_u$ so
% 				that $p_U$ can be forced from $p_I$. Compute
% 				the fixpoint of $\overline{\post}$ on it, and
% 				set it to be $p_R \in P$.
% 		\end{enumerate}
% 	\item Add more single latch predicates to $P$ and go back to the second
% 		step.
% \end{enumerate}

% The inner loop corresponds to the exhaustion of the information one can gather
% from a fixed set of predicates. Even if the initial configuration is indeed
% contained in the fixpoint of $\upreover$, one can then over-approximate the
% configurations that are \emph{reachable if \adam can force error
% configurations}. This reduces the set of configurations to be considered.

\subsubsection{Optional optimizations}
We have implemented a version of the classic fixpoint computation which receives
as input some reachability information and uses it to minimize the size of the
BDDs handled. More specifically, we choose $k$ different subsets of $L$ which we
use as predicates. Then, on this abstraction, we compute the greatest fixpoint
of $\overline{\post}$ from $p_I$. This yields $k$ over-approximations of the set
of reachable configurations of the system. After each $\upre$ operation we
\texttt{restrict} the result with each one of these over-approximations. The
\texttt{restrict} procedure is used to minimize the size of a BDD using an
additional ``don't care'' BDD (see, e.g.~\cite{hbbm97}). We assume that
\texttt{restrict} is ``safe'', that is, if the operation increases the size of
the BDD then the result is dropped in favor of the original BDD.

\subsubsection{A word on synthesis}
Denote by $\upre^*(\calU)$ the fixpoint of $\upre$ on $\calU$.
We have $\gamma(W_u) \subseteq \upre^*(\calU)$, so $\gamma(W_u)^c$ is an
over-approximation of desired set. Then $\upre^*(\gamma(W_u))^c$ gives
the set of configurations from which \eve can ensure the safety property holds.

%As a final optimization, we describe how we use \texttt{restrict} in the final
%phase of the synthesis algorithm to minimize the synthesized circuit size.

Finally, after extracting the desired circuit, which we describe by formulae $f_c(L,X_u)$
for all $c \in X_c$, one can launch a last reachability analysis. Namely, we
compute the reachable configurations of the latches when allowing only
transitions that agree with $\bigwedge_{c \in X_c} c' \Leftrightarrow f_c(L,X_u)$.
The resulting set of valuations of $L$ can be used to \texttt{restrict} all
$f_c(L,X_u)$ formulae.

\subsubsection{Experimental results (comparison of standard and abstraction-based method)}
\label{sec:experiments-discussion}
\begin{figure}
    \includegraphics[width=0.45\textwidth]{img/real-sorted-log.png}
    \caption{Time (in seconds) to check realizability.}
    \label{fig:real-sorted}
\end{figure}
% \begin{figure}
%   \includegraphics[width=0.45\textwidth]{img/real-cnt-sorted.png}
%   \caption{Time (in seconds) for \emph{cnt} benchmarks.}
%   \label{fig:real-cnt}
% \end{figure}
% \begin{figure}
%   \includegraphics[width=0.45\textwidth]{img/synth.png}
%   \caption{Size of the synthesized strategy.}
%   \label{fig:synth}
%   %\vspace{-4em}
% \end{figure}
We evaluated four different algorithms: 
\begin{inparaenum}
	\item[(C)] the classical fixpoint computation with a precomputed
		transition relation;
	\item[(C-TL)] the classical fixpoint computation using the partitioned
		transition relation and using substitution;
  % $\upre$ without a transition relation (i.e. using substitution instead);
	\item[(A)] the algorithm~\ref{alg:abs_synth} with a precomputed abstract
		transition relation;
	\item[(A-TL)] the algorithm~\ref{alg:abs_synth} using abstract operators
		implemented to avoid using a transition relation (this implies
		$\overline{\post}$ was used instead of the exact $\post$
		operator).
\end{inparaenum}
The benchmarks that we used for the evaluation are provided for the SyntComp
(Synthesis Competition) \texttt{https://syntcompdb.iaik.tugraz.at/}.  At the time
of submission of this work, there were $432$ benchmarks provided by the
organizers of the competition. We have submitted $102$ \sj{100?} additional benchmarks. 

\figurename~\ref{fig:real-sorted} summarizes performances of the algorithms on
all our benchmarks.  The horizontal axis is the number of instances that can be
solved within the time limit given by the vertical axis.  In general C-TL
performs better, however the algorithms that use abstraction perform better on
some examples.  This is in particular the case for the ``cnt'' benchmark, as can
be seen in \figurename~\ref{fig:real-cnt}.  In these benchmarks, there is a
counter (its size depends on the benchmark), the adversary can increment it and
the controller should reset it at the right moment.  The set of reachable states
is enormous but the winning strategy is quite simple which may explain why
abstraction works better. The abstract algorithms were able to solve more of
these examples within the time limit of $500$s that we fixed.

In \figurename~\ref{fig:synth} we compared the size of the synthesized circuits
with the size of the input circuits for the different sets of benchmarks.  Most
of the time, our method allows to find solutions that are not too big when
compared to the input circuit.

It is worth mentioning that from the $534$ benchmarks considered, we were able
to determine realizability in under $500$s for all but less than $30$ of them.
Amongst these, $369$ are known to be realizable. We were able to synthesize a
circuit, again in under $500$s, for all but less than $35$.


%\paragraph{The specification.}
%AbsSynthe takes as input a \emph{synchronous sequential circuit} given with a
%safety specification described by a file in the \emph{extended AIGER
%format}~\cite{SYNTCOMP-format}.
%%We are interested in synthesizing controllers for \emph{synchronous sequential
%%circuits} given with safety specifications.
%Such circuits consists of a set $L$
%of latches, a set $X_c$ of \emph{controllable} inputs, and a set $X_u$ of
%uncontrollable inputs. $\out$ is a distiguished latch which indicates if an
%error has ocurred. For each latch $l\in L$, $f_l \colon \mathbb{B}^{X_u} \times
%\mathbb{B}^{X_c} \times \mathbb{B}^L \to \mathbb{B}$ is the \emph{transition
%function} that gives the valuation of $l$ in the next step. 

%A \emph{synchronous sequential circuit} is a tuple $\langle
%X_u, X_c, L, (f_l)_{l\in L}, \fbad \rangle$,
%Intuitively,
%controllable inputs are to be determined by the controller to be synthesized,
%while uncontrollable inputs cannot be restricted, and are determined by the
%environment. 
%We assume that the safety specifications are embedded in the circuit; more
%precisely,
%A distinguished latch indicates if an error has
%occurred. Formally, a \emph{synchronous sequential circuit} is a tuple $\langle
%X_u, X_c, L, (f_l)_{l\in L}, \fbad \rangle$, where:
%\begin{itemize}
%	\item $X_u, X_c, L$ are finite sets of boolean variables representing
%		\emph{uncontrollable inputs}, \emph{controllable inputs}, and
%		\emph{latches} respectively;
%	\item for each latch $l\in L$, $f_l \colon \mathbb{B}^{X_u} \times
%		\mathbb{B}^{X_c} \times \mathbb{B}^L \to \mathbb{B}$ is the
%		\emph{transition function} that gives the valuation of $l$ in
%		the next step; 
%	\item $\fbad$ is the \emph{error function} $\fbad \colon
%		\mathbb{B}^{X_u} \times \mathbb{B}^{X_c} \times \mathbb{B}^L \to
%		\mathbb{B}$, which evaluates to true in error configurations. 
%\end{itemize}
%
%Given a circuit, our goal is to synthesize a \emph{controller} which, given any
%valuation of the latches and uncontrollable inputs, sets the controllable
%inputs, in order to ensure that the overall system never enters an error
%configuration.

\noindent
{\bf Tool availability.}
The tool itself is available at \url{https://github.com/gaperez64/AbsSynthe}. It
is mostly Python code. It depends only on a simple AIG library (fetched
from~\cite{aiger}) and the CUDD binary decision diagram package~\cite{somenzi99}.


==> analysis.tex <==
\section{Analysis of Results}
\label{sec:analysis}
\sj{is it a good idea to separate results and analysis?}
\sj{probably not, join them again.}

\subsection{Realizability Track}

As can be seen in Figures~\ref{fig:rs-cactus} and \ref{fig:rp-cactus}, most 
tools have a very steep degradation with higher complexity of benchmarks, 
i.e., between $90\%$ and $95\%$ of the benchmarks that can be solved within 
the timeout of $5000$ seconds can actually be solved very quickly, i.e., in 
less than $600$ seconds. The degradation is more graceful for the learning-
based approach of Demiurge, but this approach solves fewer problems overall 
than the BDD-based approaches.

\subsubsection{Sequential Subtrack}
We note that in our ranking Demiurge (learn) has the same 
score as Basil (and higher than AbsSynthe), even though it can only solve $359$
problems, compared to $520$ for Basil and $536$ for AbsSynthe. This 
is because Demiurge is very fast for small problem instances, and for 
problems that it does solve, it is often the fastest of all tools.

The uniquely solved benchmarks show that there are significant differences 
between the algorithms of different tools. In particular, the template-based 
variant of Demiurge, while not very successful overall, can determine 
realizability for a number of toy examples that are simple in idea, and only 
become complex due to the choice of a sufficiently large parameter.


\subsubsection{Parallel Subtrack}
Concerning the effectiveness of parallel versus sequential implementations of 
realizability checkers, this subtrack shows that currently none of the 
implementations benefits substantially from useing parallelism. To the 
contrary, the best-performing tool is a sequential implementation, and the 
parallel implementations of Demiurge and Realizer(?) were not able to solve 
(in 5000s Wall Time) the problems that their sequential implementations solved 
uniquely in the sequential subtrack (in 5000s CPU Time). 

Furthermore, the different ranking of purely sequential tools in the parallel 
and sequential subtracks shows a weakness of our ranking system: assigning 
points for the relative rank in time needed to solve any given problem 
heavily favors implementations in C++ that have a quick startup time. Basil 
and Demiurge solve 150 and 100 problems, respectively, in less than $0.36$s 
Wall Time, which is the minimal time needed to solve any single problem for 
the Python-based implementations AbsSynthe and Realizer. 

Summing up, the ranking scheme together with the selection of benchmarks 
favors tools that can solve easy benchmarks very quickly, and in particular 
tools implemented in C++, as they make very efficient use of Wall Time, 
compared to Python-based tools.

\subsection{Synthesis Track}

\subsubsection{Sequential Subtrack}
Note that the score of Basil is much lower than that of Demiurge, even though 
almost as many benchmarks are solved and checked. This is because in many 
cases the SAT-based approach of Demiurge 
provides smaller implementations (that are ranked higher) than the BDD-based 
approaches of AbsSynthe and Basil. Figure~\ref{fig:size-ss2} shows that for 
those instances of the AMBA and GenBuf benchmarks that Demiurge (learn) can 
solve, it provides implementations that are often by an order of magnitude 
smaller than those of the other tools. However, as shown in 
Figures~\ref{fig:size-ss1} , there is also a substantial number of benchmarks 
where the implementation sizes are equal or very similar.

Furthermore, we note that the benchmark set contains 
relatively many problems that are easy to solve. For example, AbsSynthe can 
solve $75$ of the $157$ problems in less than $0.5$s CPU Time. Demiurge 
profits from the fact that there are not many hard benchmarks, and that it 
provides the smallest or at least one of the smallest implementations for the 
benchmarks that it can solve.

Comparing AbsSynthe and Basil, the former 
seems to implement optimizations that allow it to solve larger problems and 
come up with smaller solutions in many cases. \sj{probably partitioned 
transition relation?}

\subsubsection{Parallel Subtrack}

In the parallel subtrack, Demiurge profited from the combination of its 
learning- and template-based approaches. While it solved $2$ problems less 
than the best single strategy (learning) in the sequential subtrack, its 
solutions were in some cases even smaller, effectively ranking it higher than 
AbsSynthe, which solved more problems but provided solutions of lower quality.
